OstQuant: Refining Large Language Model Quantization with Orthogonal and Scaling Transformations for Better Distribution Fitting

Post-training quantization (PTQ) has emerged as a widely adopted technique for compressing and accelerating Large Language Models (LLMs). The major challenge in LLM quantization is that uneven and heavy-tailed data distributions can expand the quantization range, thereby reducing bit precision for most values. Recent methods attempt to eliminate outliers and balance inter-channel differences by employing linear transformations; however, they remain heuristic and are often overlook optimizing the data distribution across the entire quantization space.In this paper, we introduce Quantization Space Utilization Rate (QSUR), a novel metric that effectively assesses the quantizability of transformed data by measuring the space utilization of the data in the quantization space. We complement QSUR with mathematical derivations that examine the effects and limitations of various transformations, guiding our development of Orthogonal and Scaling Transformation-based Quantization (OSTQuant). OSQuant employs a learnable equivalent transformation, consisting of an orthogonal transformation and a scaling transformation, to optimize the distributions of weights and activations across the entire quantization space. Futhermore, we propose the KL-Top loss function, designed to mitigate noise during optimization while retaining richer semantic information within the limited calibration data imposed by PTQ. OSTQuant outperforms existing work on various LLMs and benchmarks. In the W4-only setting, it retains 99.5\% of the floating-point accuracy. In the more challenging W4A4KV4 configuration, OSTQuant reduces the performance gap by 32\% on the LLaMA-3-8B model compared to state-of-the-art methods. \href{https://github.com/BrotherHappy/OSTQuant}{https://github.com/BrotherHappy/OSTQuant}.

==> figs/1_smooth_r_ours.tex <==
\begin{figure}[!htbp]
    \subfigure[Original]{
       \centering
        \includegraphics[width=0.24\textwidth]{figs/Fig1_a.png}
    \label{Fig1 a}
    }\subfigure[Smooth Transform]{
        \centering
        \includegraphics[width=0.24\textwidth]{figs/Fig1_b.png}
        \label{Fig1 b}
    }\subfigure[Rotation Transform]{
        \centering
        \includegraphics[width=0.24\textwidth]{figs/Fig1_c.png}
        \label{Fig1 c}
    }\subfigure[Ours]{
        \centering
            \includegraphics[width=0.24\textwidth]{figs/Fig1_d.png}
        }
        \label{Fig1 d}
    % \hspace{+15pt}
       \vspace{-2mm}
        \caption{
        Transformation of a batch of data $X \sim \mathcal{N}(\bm{\mu}, \bm{\Sigma})$  using different methods. Eigenvalues  $\lambda_1$  and  $\lambda_2$  represent the spread of the distribution along principal axes after eigenvalue decomposition of  $\Sigma$ . (a) shows the original distribution, while (b), (c), and (d) illustrate the effects of the Smooth-based, Rotate-base, and ours OST-based methods, respectively, on QSUR.} 
        \label{Fig abcd}
        % \vspace{-7mm}
\end{figure}
    

==> figs/3-4.tex <==
\begin{figure}[thb]
  \begin{minipage}[b]{0.47\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/3_1_DistributionBeforeAfterOSTQuant.png}
    \caption{Activation distribution in the LLaMA-3-8B before and after applying OSTQuant shows significant differences. Prior to transformation, the distribution across different channels exhibits substantial variation and contains numerous outliers. After OSTQuant, the distributions become more uniform across channels.}
    \label{Fig3}
    \label{Fig act dist}
  \end{minipage}%
  \hspace{20pt}
  \begin{minipage}[b]{0.47\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/3_2_QSUR_Score.png}
    \caption{Zero-Shot$^9$ precision retention (under W4A4 quantization) and normalized QSUR are evaluated for LLaMA variants across different quantization methods. The normalized QSUR is derived as the $d$-th root of QSUR, where $d$ denotes the number of channels. QSUR exhibits a positive correlation with accuracy.}
    \label{Fig4}
    \label{Fig qsur score}
  \end{minipage}
  \vspace{-3mm}
\end{figure}

% \begin{figure}[h]
%   \begin{minipage}[b]{0.48\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/3_1_DistributionBeforeAfterOSTQuant.png}
%         \caption{Activation distribution in the LLaMA-3 8B model before and after applying OSTQuant show significant differences. Prior to transformation, the distribution across different channels exhibit substantial variation and contain numerous outliers. After OSTQuant, the distributions become more uniform across channels.}
%         \label{Fig3}
%   \end{minipage}%
%   \hspace{2pt}
%   \begin{minipage}[b]{0.48\linewidth}\label{Fig4}
%     \centering
%     \includegraphics[width=\linewidth]{figs/3_2_QSUR_Score.png}
%         \caption{Zero-shot precision retention(under W4A4 quantization) and normalized QSUR are evaluated for LLaMA variants across different quantization methods. The normalized QSUR is derived as the d-th root of QSUR, where d denotes the number of channels. QSUR exhibits a positive correlation with accuracy.}
%         \label{Fig4}
%   \end{minipage}
%   \vspace{-3mm}
% \end{figure}


==> figs/5_MainMethod.tex <==
\begin{figure}[htbp]
\vspace{-4mm}
\centering
\begin{minipage}[t]{\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/FigMainMethod.png}
        \caption{Details of OSTQuant. In the top section demonstrates how the global orthogonal transformation $\bm{R}_{res}$, together with the two diagonal transformations, $\bm{S}_{attn}$ and $\bm{S}_{ffn}$, within each block, jointly act on the linear layers in residual connections to achieve distribution adjustment across the entire network. The bottom section highlights how four sets of identical diagonal and scaling transformations in the Self-Attention and FFN networks are combined with the weights to facilitate block-wise distribution adjustment.}
    \label{Fig MainMethod}
\end{minipage} \vspace{-2mm}
\vspace{-2mm}
\end{figure}
\vspace{-1mm}

==> figs/6-7_illext-tokendiff.tex <==
\begin{wrapfigure}{r}{0.50\linewidth}  % 'r' 表示图在右侧, 宽度为50%
    \centering
    \vspace{-20mm}
    \includegraphics[width=\linewidth]{figs/token_difference.png}
    \vspace{-8mm}
    \caption{The distribution of the number of tokens required to accumulate 90\% of the total prediction probability in the LLaMA-2-7B.}
    \label{Fig7}
    \vspace{-5mm}
\end{wrapfigure}
